A baseline correction algorithm for FAST

The Five-hundred-meter Aperture Spherical radio Telescope (FAST) is the most sensitive ground-based, single-dish radio telescope on Earth. However, the original HI spectra produced by FAST are affected by standing waves. To maximize the power of FAST for high-sensitivity observations, we proposed an algorithm that combines fast Fourier transforms and extreme envelope curves to automatically correct the baselines of FAST HI spectra and remove standing waves from the baselines. This algorithm can reduce the amplified noise level caused by standing waves to a near-ideal level without losing signals or introducing false signals. The root mean square of the average baseline reaches $\sim$ 8 mK, approaching the theoretical sensitivity of an HI spectrum produced by FAST for an integration time of 335 minutes, i.e., $\sim$ 6 mK.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

